Large-Scale Analysis of Online Questions Related to Opioid Use Disorder on Reddit

Opioid use disorder (OUD) is a leading health problem that affects individual well-being as well as general public health. Due to a variety of reasons, including the stigma faced by people using opioids, online communities for recovery and support were formed on different social media platforms. In these communities, people share their experiences and solicit information by asking questions to learn about opioid use and recovery. However, these communities do not always contain clinically verified information. In this paper, we study natural language questions asked in the context of OUD-related discourse on Reddit. We adopt transformer-based question detection along with hierarchical clustering across 19 subreddits to identify six coarse-grained categories and 69 fine-grained categories of OUD-related questions. Our analysis uncovers ten areas of information seeking from Reddit users in the context of OUD: drug sales, specific drug-related questions, OUD treatment, drug uses, side effects, withdrawal, lifestyle, drug testing, pain management and others, during the study period of 2018-2021. Our work provides a major step in improving the understanding of OUD-related questions people ask unobtrusively on Reddit. We finally discuss technological interventions and public health harm reduction techniques based on the topics of these questions.

==> SectionFiles/metadata.tex <==
\section*{Author Contributions}
 Sumner and De Choudhury designed the research; ElSherief, Sumner, and De Choudhury conceptualized and developed the analytic techniques; ElSherief gathered and analyzed the data and designed the Machine Learning models; Sumner, Jones, Law, Kacha-Ochana, Schieber, Cordier, and Holton provided expert clinical review and/or annotations for the models and read, edited, and provided feedback on the paper; ElSherief, Sumner, and De Choudhury interpreted the results and drafted the paper.
 
 
%  ElSherief
%  Sumner
%   Jones, 
%   Law, 
%   Kacha-Ochana
%   Schieber
%   Cordier
%   Holton
%   De Choudhury
  
 

\section*{Acknowledgments/Funding}
This research was supported through a contract by the CDC (via the Department of Health and Human Services) to the Georgia Institute of Technology (PI: Munmun De Choudhury). CDC investigators participated in the design and conduct of the study; collection, management, analysis, and interpretation of the data; preparation, review, or approval of the manuscript; and decision to submit the manuscript for publication. ElSherief and De Choudhury had full access to all the data in the study and take responsibility for the integrity of the data and the accuracy of the data analysis. We thank Kenneth Kannampully for his help with the Drugs-Forum.com data collection.

\section*{Declaration of Interests}
We declare no competing interests.

\section*{CDC Disclaimer}
The findings and conclusions in this report are those of the authors and do not necessarily represent the official position of the Centers for Disease Control and Prevention.












